$s$-Modular, $s$-congruent and $s$-duplicate partitions

In this paper, we investigate the combinatorial properties of three classes of integer partitions: (1) $s$-modular partitions, a class consisting of partitions into parts with a number of occurrences (i.e., multiplicity) congruent to $0$ or $1$ modulo $s$, (2) $s$-congruent partitions, which generalize Sellers' partitions into parts not congruent to $2$ modulo $4$, and (3) $s$-duplicate partitions, of which the partitions having distinct odd parts and enumerated by the function $\mypod(n)$ are a special case. In this vein, we generalize Alladi's series expansion for the product generating function of $\mypod(n)$ and show that Andrews' generalization of G\"ollnitz-Gordon identities coincides with the number of partitions into parts simultaneously $s$-congruent and $t$-distinct (parts appearing fewer than $t$ times).

==> sn-bibliography.tex <==
\begin{thebibliography}{24}

\bibitem{r1} K. Alladi, Partitions with non-repeating odd parts and $q$-hypergeometric identities. \textit{The legacy of Alladi Ramakrishnan in the mathematical sciences}, Springer, New York, NY. (2010), 169--182.

\bibitem{All1} K. Alladi, Partition identities involving gaps and weights. \textit{Trans. Am. Math. Soc.} \textbf{349} (1997),
5001-5019.

\bibitem{All2} K. Alladi, A combinatorial correspondence related to G\"ollnitz's (Big) partition theorem and
applications. \textit{Trans. Am. Math. Soc.} \textbf{349} (1997), 2721--2735.

\bibitem{r2} G. E. Andrews, A generalization of the G\"ollnitz-Gordon partition theorems. \textit{Proc. Am. Math. Soc.} \textbf{18} (1967), 945--952.

\bibitem{r3} G. E. Andrews, Two theorems of Gauss and allied identities proved arithmetically. \textit{Pac. J. Math.} \textbf{41} (1972), 563--578.

\bibitem{r4} G. E. Andrews, K. Alladi, and B. Gordon, Generalizations and refinements of a partition theorem of G\" ollnitz. \textit{J. Reine Ang. Math.} \textbf{460} (1995), 165--188.

\bibitem{ANDB} G. E. Andrews, The theory of partitions. \textit{Encyclopedia of Math. and its Applications} \textbf{2} (1976), Addison Wesley.

\bibitem{r5} A. Berkovich, F. G. Garvan, Some observations on Dyson's new symmetries of partitions. \textit{J. Comb. Theory, Ser. A} \textbf{100} (2002), 61--93.

\bibitem{r6} S. P. Cui, N. S. Gu, Arithmetic properties of $\ell$-regular partitions. \textit{Adv. Appl. Math.} \textbf{51} (2013), 507--523.

\bibitem{COR} S. Corteel, J. Lovejoy,  Overpartitions. \textit{Trans. Amer. Math. Soc.} \textbf{365} (2003), 623--635.

\bibitem{r7} B. Dandurand, D. Penniston, $\ell$-divisibility of $\ell$-regular partition functions. \textit{Ramanujan J.} \textbf{19} (2009), 63--70. 

\bibitem{r8} B. Drake, Limits of areas under lattice paths. \textit{Discrete Math.} \textbf{309} (2009), 3936--3953.

\bibitem{r10} L. Ferrari, Schr\"oder partitions, Schr\"oder tableaux and weak poset patterns. \textit{Contrib. Discrete Math.} \textbf{16} (2021), 160--184.      

\bibitem{Fin} N. J. Fine, Basic hypergeometric series and applications, \textit{Math. Surveys and Monographs}
\textbf{27} (1988), Amer. Math. Soc., Providence.

\bibitem{r11} A. Fink, R. Guy,  M. Krusemeyer, Partitions with parts occurring at most thrice. \textit{Contrib. Discrete Math.} \textbf{3} (2008).

\bibitem{GOL} H. G\" ollnitz, Partitionen mit Differenzenbedingungen. \textit{Journal f\"ur die reine und angewandte Mathematik} \textbf{225} (1967), 154--190.

\bibitem{GOR} B. Gordon, Some Continued Fractions of the Rogers-Ramanujan Type. \textit{Duke Mathematical Journal} \textbf{32} (1965), 741--748.

\bibitem{r12} P. Hagis, Partitions with a restriction on the multiplicity of the summands. \textit{Trans. Amer. Math. Soc.} \textbf{155} (1971), 375--384.

\bibitem{r13} M. D. Hirschhorn, J. A. Sellers, Arithmetic properties of partitions with odd parts distinct. \textit{Ramanujan J.} \textbf{22} (2010), 273--284.

\bibitem{r14} D. Kim, A. J. Yee, A Note on Partitions into Distinct Parts and Odd Parts. \textit{Ramanujan J.} \textbf{3} (1999), 227--231.

\bibitem{r15} J. Lovejoy, R. Osburn, Quadratic forms and four partition functions modulo $3$. \textit{Integers} \textbf{11} (2011), Paper A4.

\bibitem{r16} M. Merca, On the partitions into distinct parts and odd parts. \textit{Quaest. Math.}, \textbf{44} (2021), 1095--1105.

\bibitem{r17} M. Merca, On the number of partitions into parts not congruent to $0$, $\pm 3 $ (mod  $12$). \textit{Period. Math. Hung.} \textbf{83} (2021), 133--143.

\bibitem{r18} M. Merca, New relations for the number of partitions with distinct even parts. \textit{J. Number Theory} \textbf{176} (2017), 1--12.

\bibitem{r19} S. Radu, J. A. Sellers, Congruence properties modulo $5$ and $7$ for the pod function. \textit{Int. J. Number Theory}, \textbf{7} (2011), 2249--2259.

\bibitem{Syl} J. J. Sylvester, A constructive theory of partitions in three Acts, an Interact, and an Exodion.
\textit{Am. J. Math.} \textbf{5} (1882), 251--330.

\bibitem{r20} A. Sills, Rademacher-type formulas for restricted partition and overpartition functions. \textit{Ramanujan J.} \textbf{23} (2010), 253--264.

\bibitem{r21} Sloane, N.: The On-Line Encyclopedia of Integer Sequences. Published electronically at  https://oeis.org, 2024.

\bibitem{r22} D. Spector, Duality, partial supersymmetry, and arithmetic number theory. \textit{J. Math. Phys.} \textbf{39} (1998), 1919--1927.

\bibitem{r23} L. Wang, New Congruences for Partitions where the Odd Parts are Distinct. \textit{J. Integer Seq.} \textbf{18} (2015), Article 15.4.2.

\bibitem{r24} M. P. Zaletel, R. S. Mong, Exact matrix product states for quantum Hall wave functions. \textit{Phys. Rev. B}  \textbf{86} (2012), 245--305.

\bibitem{Zen} J. Zeng, The q-variations of Sylvester's bijection between odd and strict partitions.
\textit{Ramanujan J.} \textbf{9} (2005), 289--303.

\end{thebibliography}


